Self-Evolving Agents through Privileged Retrospective Distillation

Self-evolving agents aim to improve from their own experience rather than remain fixed after deployment, but naturally collected trajectories often lack ground-truth solutions or verifier-derived rewards. We introduce Retrospective Self-Distillation (RSD), a multi-round framework that turns such experience into dense supervision using privileged retrospective context. For each on-policy trajectory, the same underlying model acts as both student and teacher: the teacher re-scores the student's realized actions while conditioning on cross-task precedents and lessons, together with turn-level reflection and future hindsight from the completed trajectory. The resulting teacher distribution is distilled back into the policy through on-policy self-distillation. Across rounds, the experience bank grows and the retrospective context is refreshed, allowing the model, its data, and its supervision to co-evolve. We further introduce frontier-guided context-policy evolution, where a stronger frontier model proposes constrained edits to how privileged context is constructed. Across ALFWorld, ScienceWorld, and SearchQA with Qwen3-8B and Qwen3-14B, RSD improves performance by up to 59.7% relative to the base model, while frontier-guided context-policy evolution adds up to a further 44.7% relative improvement over a fixed context policy. These results show that naturally accumulated experience can be converted into persistent model capability without ground-truth trajectories or verifier-derived rewards for the core policy update.

==> neurips_sections/0_abstract.tex <==
Self-evolving agents aim to improve from their own experience rather than remaining fixed once deployed.
%
In practice, however, naturally collected agent trajectories often lack ground-truth solutions or verifier-derived rewards, making them difficult to learn from.
%
We observe that these trajectories become substantially more informative in \textit{retrospect}. 
%
When the agent takes an action, it knows only what has happened so far, but looking back after the trajectory ends, the same action can be judged with knowledge the agent lacked at that moment, including how the environment responded afterward and how related tasks in its accumulated experience succeeded or failed.
%
Based on this observation, we introduce \textbf{Retrospective Self-Distillation (\ours)}, a multi-round self-evolution framework 
%
in which the same model, given privileged retrospective context built from its own experience, acts as a teacher that re-scores its own actions, and the resulting distribution is distilled back into the policy through on-policy self-distillation.
%
The privileged context combines cross-task precedents and lessons with turn-level reflection and future hindsight, allowing both successful and imperfect trajectories to provide dense supervision.
%
%
\ours is also built to make this supervision improve alongside the agent.
%
Every round, precedents and lessons are re-derived from the experience bank enlarged with the current policy's trajectories, and reflection and hindsight are computed fresh for each new trajectory, so the teacher always scores the policy against its most recent experience.
%
We further introduce \textit{frontier-guided context-policy evolution}, 
in which a stronger frontier model proposes edits to the context construction rules, for example how many precedents to retrieve or which components to include.
%
Across ALFWorld, ScienceWorld, and SearchQA with Qwen3-8B and 14B, \ours improves performance by up to $59.7\%$ relative over the base model, and frontier-guided context-policy evolution adds up to a further $44.7\%$ relative improvement over a fixed context policy.
%
These results show that agents can convert naturally accumulated experience into persistent model capability without ground-truth trajectories or verifier-derived rewards for the core policy update.

==> neurips_sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Large language model (LLM) agents are increasingly capable of interacting with complex environments and completing multi-turn tasks.
%
Yet most agents remain largely fixed after post-training: the substantial interaction experience generated during deployment does not automatically translate into persistent improvements in the underlying model.
%
This has motivated growing interest in \emph{self-evolving agents}, which aim to establish a closed-loop \emph{data flywheel} where the current policy generates on-policy interaction experience, learns from that experience, and then produces increasingly useful data in subsequent rounds~\citep{gao2025survey}.
%
Prior approaches pursue this goal either by evolving external components such as prompts, workflows, memory, or tools~\citep{hu2025automated}, or by adapting model parameters using successful trajectories, supervised learning, or reinforcement learning~\citep{zhai2025agentevolver}.
%
However, these approaches often assume supervision that may not be naturally available during agent interaction.

In practical settings, each task may yield only a single on-policy trajectory, without a ground-truth trajectory specifying what the agent should have done or a reliable verifier providing rewards for policy optimization.
%
Conventional supervised fine-tuning therefore lacks direct target sequences, while verifier-based reinforcement learning requires reliable rewards or additional exploration to identify successful behavior~\citep{wu2026seed}.
%
Restricting training to successful trajectories further discards much of the already collected experience, including failures that may contain informative environment feedback.
%
This raises a central question: \emph{How can an agent continuously improve from its naturally accumulated interaction experience without requiring ground-truth trajectories or verifier-derived rewards for policy optimization?}

Our key observation is that although such trajectories may lack explicit training targets, they become substantially more informative \emph{after} the interaction has completed.
%
For the current task, downstream environment observations reveal the consequences of earlier decisions and provide hindsight unavailable when those actions were taken.
%
Across tasks, accumulated past experience provides concrete precedents, reusable strategies, and recurring failure patterns.
%
We therefore construct a \emph{privileged retrospective view} of each agent decision by combining information from both the completed current trajectory and accumulated prior experience.
%
This information asymmetry naturally matches on-policy self-distillation (OPSD): the same underlying model acts as both student and teacher, while the teacher retrospectively receives privileged information unavailable to the student during rollout.~\citep{zhao2026self}.
%
Unlike conventional OPD, which relies on a separate teacher~\citep{agarwal2024policy}, our setting constructs privileged supervision directly from the agent's own evolving interaction experience.

Based on this observation, we introduce \ours, a multi-round self-evolution framework that couples on-policy experience collection with privileged retrospective distillation.
%
At each round, the current policy generates new trajectories and incorporates them into an accumulated experience bank.
%
For every interaction turn, privileged context combines \emph{precedents} from related past experience, \emph{lessons} distilled from accumulated successes and failures, \emph{reflection} on the current decision, and \emph{future hindsight} from downstream interaction and environment feedback.
%
The privileged teacher retrospectively re-scores the student's realized actions under this richer view, and the resulting supervision is distilled back into the policy.
%
As this process repeats, the model, its on-policy experience, and the privileged context constructed from that experience evolve together.
%
We further explore a stronger-access extension, \emph{frontier-guided context-policy evolution}, in which a frontier model also adapts how privileged context is constructed, yielding a self-evolution loop over both model capability and retrospective supervision.

We evaluate \ours with various models across ALFWorld, ScienceWorld, and SearchQA.
%
\ours yields up to a $59.7\%$ relative improvement over the base model on ScienceWorld, while frontier-guided context-policy evolution provides a further relative gain of $44.7\%$ over the fixed context policy.
%
% We also find strong gains on ALFWorld, whereas SearchQA remains within a narrow performance band across rounds, providing a complementary boundary case for behavioral self-evolution.

Our main contributions are:
\begin{itemize}[leftmargin=*]
    \item We formulate a practical self-evolving agent setting that turns naturally generated on-policy interaction experience into a recurrent data flywheel without requiring ground-truth trajectories or verifier-derived rewards for the core policy update.
    
    \item We introduce privileged retrospective distillation from accumulated experience and trajectory hindsight, and further extend it with frontier-guided context-policy evolution so that both the model and its retrospective supervision can evolve across rounds.
    
    \item Across ALFWorld, ScienceWorld, and SearchQA, \ours achieves up to $59.7\%$ relative improvement over the base model, while frontier-guided context-policy evolution yields up to an additional $44.7\%$ relative gain over the fixed context policy.
\end{itemize}

==> neurips_sections/2_related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Self-Evolving Language Agents}
Self-evolving language agents aim to continuously improve from their own interaction experience rather than remaining fixed after post-training~\citep{gao2025survey, tao2024survey}.
%
One line of work primarily evolves the external agent system, including prompts, workflows, memory, tools, and other agentic structures~\citep{hu2025automated, zhang2025aflow, li2024autoflow, wu2026remember}.
%
Automated agent-design methods search over workflow or program structures, while experience-driven agents continually refine explicit memories, reusable strategies, or dynamically constructed assets~\citep{yang2025learning, wu2025evolver, wei2025evo, cheng2026mem2evolve}.
%
These approaches demonstrate that accumulated interaction experience can improve future behavior, but much of the acquired capability remains mediated by an external scaffold rather than being persistently incorporated into the underlying policy~\citep{lee2026recursive}.

A complementary line of work directly adapts the agent model itself.
%
Recent approaches use online parameter updates, reinforcement learning, self-generated tasks, reward models, or hindsight supervision to internalize interaction experience into persistent model capability, reducing dependence on external scaffolds and enabling subsequent behavior to improve as new experience accumulates~\citep{zhai2025agentevolver, sun2025towards, ren2026scaling, wu2026seed}.
%
While these methods move self-evolution from the scaffold toward model weights, many rely on explicit verifiers, successful trajectories, or additional exploration to determine which experience should drive learning~\citep{zuo2026ttrl, zhang2026test}.
%
In contrast, we construct a data flywheel that does not use
verifier-derived rewards for the core policy update, instead distilling
privileged retrospective supervision from both the current trajectory and
accumulated interactions directly into model weights, allowing the policy
and its supervision to co-evolve across rounds.

\subsection{On-Policy Distillation and Privileged Context}
On-policy distillation (OPD) addresses the train--inference mismatch of conventional knowledge distillation by training the student on trajectories sampled from its own policy, while a teacher provides dense token-level supervision on those student-visited states~\citep{agarwal2024policy, yang2026learning, zhou2026omniopd}.
%
This formulation makes distillation naturally compatible with iterative policy improvement, since supervision is applied directly to the distribution induced by the evolving student.

Recent work extends this idea by changing what information is available to the teacher.
%
On-Policy Context Distillation (OPCD) conditions the teacher on additional context while the student generates without it, allowing useful in-context knowledge, such as historical solution traces or optimized prompts, to be internalized into model parameters~\citep{ye2026policy}.
%
On-Policy Self-Distillation (OPSD) further removes the need for a separate teacher model: the same underlying model acts as both teacher and student, with the teacher granted privileged information unavailable to the student; existing formulations commonly construct this privileged view from ground-truth solutions~\citep{zhao2026self, xu2026beta}.
%
Related self-distillation methods similarly exploit verified solutions, environment feedback, or successful rollouts as privileged signals~\citep{hubotter2026reinforcement,pan2026rlcsd,he2026self}.

In contrast, our core method requires neither ground-truth trajectories nor verifier-derived rewards for model-parameter optimization.
%
We construct privileged retrospective context from the agent's own current trajectory and accumulated prior experience, and continually refresh this context as new on-policy experience is collected, coupling context evolution with model-weight evolution.

==> neurips_sections/3_prelim.tex <==
\section{Preliminaries}\label{subsec:preliminaries}

\subsection{Self-Evolving Agents}
\label{sec:prelim_self_evolution}

We consider a multi-turn agent that improves through a sequence of self-evolution rounds.
%
At round $r$, the agent is parameterized by a policy $\pi^{(r)}$.
%
Given a task $x$, the agent interacts with the environment over multiple turns.
%
At turn $i$, it observes the interaction history $h_i$ and generates an action
\[
a_i \sim \pi^{(r)}(\cdot \mid h_i),
\]
after which the environment returns a new observation $o_{i+1}$.
%
The resulting trajectory is denoted as
\[
\tau=(x,o_1,a_1,o_2,a_2,\ldots,o_{T+1}),
\qquad
\tau\sim\pi^{(r)}.
\]
%
Collecting trajectories over a set of tasks produces the round-$r$ on-policy experience
$\mathcal{D}^{(r)}$.

We focus on a practical self-evolution setting in which each sampled task produces a single on-policy trajectory, rather than repeated attempts followed by success-based selection.
%
We further assume no ground-truth trajectories or verifier-derived rewards for policy optimization, requiring the agent to extract useful supervision directly from its naturally collected interaction experience.

A self-evolving agent iteratively updates its policy using experience generated by its current policy,
\begin{equation}
\pi^{(r+1)}
=
\mathcal{U}\!\left(
\pi^{(r)},\mathcal{D}^{(r)}
\right),
\qquad
\mathcal{D}^{(r)}\sim\pi^{(r)},
\label{eq:self_evolution}
\end{equation}
where $\mathcal{U}$ denotes a generic self-improvement procedure.
%
Because $\pi^{(r+1)}$ induces a new interaction distribution, subsequent rounds continuously generate new on-policy experience for further improvement.
%
This iterative coupling between policy evolution and experience generation provides the basis for a self-evolving data flywheel.
%
In the following, we instantiate $\mathcal{U}$ using on-policy self-distillation.

\subsection{On-Policy Self-Distillation}
\label{sec:prelim_opsd}

On-policy self-distillation (OPSD) learns from trajectories generated by the current policy rather than from a fixed offline dataset.
%
The policy $\pi^{(r)}$ generates an on-policy trajectory
$\tau \sim \pi^{(r)}$.
%
OPSD uses the same underlying model to instantiate both student and teacher, with the teacher additionally receiving privileged retrospective context unavailable when the action was generated.
%
For a multi-turn agent, this privileged information is constructed at the turn level.
%
Let $c_i^{(r)}$ denote the privileged context for interaction turn $i$, and let $h_{i,j}$ denote the interaction history together with the generated action prefix preceding token $j$ at that turn.
%
The corresponding student and teacher distributions are
\[
\pi^{(r)}(\cdot \mid h_{i,j})
\qquad \text{and} \qquad
q^{(r)}(\cdot \mid h_{i,j},c_i^{(r)}),
\]
respectively, where $\pi^{(r)}$ and $q^{(r)}$ represent the unprivileged and privileged views of the underlying model.

The student is trained to match the privileged teacher distribution on its own on-policy states.
%
Aggregating token-level supervision across interaction turns gives
\begin{equation}
\mathcal{L}_{\mathrm{OPSD}}^{(r)}
=
\mathbb{E}_{\tau \sim \pi^{(r)}}\!
\left[
\sum_i \sum_j
D_{\mathrm{KL}}
\left(
q^{(r)}(\cdot \mid h_{i,j},c_i^{(r)})
\,\|\, 
\pi_{\theta}(\cdot \mid h_{i,j})
\right)
\right].
\label{eq:opsd}
\end{equation}
%
Because supervision is evaluated directly on the states visited by the current policy, OPSD can learn from imperfect and unsuccessful trajectories without requiring a ground-truth action sequence for each state.
%
After optimization, the resulting student becomes the policy $\pi^{(r+1)}$ for the next self-evolution round.

==> neurips_sections/4_method.tex <==
\section{\ours}\label{sec:workflow}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/method_overview.png}
    \caption{
    Overview of \ours.
    %
    At self-evolution round $r$, the current policy $\pi^{(r)}$ first collects on-policy interaction experience, which is incorporated into the accumulated experience bank.
    %
    Privileged retrospective context is then constructed from past experience: precedents and lessons, together with reflection and future hindsight from the completed current trajectory.
    %
    The same underlying model retrospectively re-scores the student's realized actions under this privileged view, and the resulting distribution is distilled back into the student to obtain $\pi^{(r+1)}$.
    %
    Repeating this process jointly evolves the policy, accumulated experience, and retrospective supervision.
    %
    In the stronger-access extension, a frontier model additionally adapts the context-construction policy $\phi^{(r)}$ across rounds.
    }
    \label{fig:method_overview}
\end{figure}

Our goal is to build a self-evolving training pipeline in which an agent repeatedly generates on-policy interaction experience, learns from that experience, and uses the improved policy to produce increasingly useful data in subsequent rounds.
%
In the absence of ground-truth trajectories or reliable verifier-derived rewards, however, it is difficult to directly convert these rollouts into supervision through conventional supervised fine-tuning (SFT) or reward-based reinforcement learning (RLVR).
%
Nevertheless, the collected experience contains rich information that becomes available retrospectively: for the current task, the completed trajectory provides downstream environment feedback and interaction outcomes, while previous tasks contribute accumulated successful and failed experiences.
%
These signals provide a richer view of the agent's behavior than was available at action time.

This observation naturally motivates OPSD.
%
Rather than requiring an external target trajectory or scalar reward, we construct privileged retrospective context from the agent's accumulated experience and use it to re-score the agent's own on-policy trajectory.
%
The resulting privileged teacher distribution provides dense supervision on exactly the states visited by the current policy, which is then distilled back into the agent to produce the next generation.
%
As this process repeats, the evolving policy generates new experience that refreshes the privileged context, forming a data flywheel between model capability, interaction experience, and retrospective supervision.
%
Algorithm~\ref{alg:self_evolution} in \appref{sec:self_evolution_algorithm}
summarizes the complete agent self-evolving procedure.

\subsection{Self-Evolution through Privileged Retrospective Distillation}
\label{sec:self_evolution_method}

An overview of the complete self-evolution framework is shown in \figref{fig:method_overview}.
%
Our self-evolution pipeline alternates between on-policy experience collection and model update across rounds.
%
We use this round-based design so that each update is trained on trajectories sampled from a fixed current policy, after which the updated policy generates a refreshed on-policy distribution for the next round.
%
At round $r$, the current policy $\pi^{(r)}$ interacts with the environment and collects a new trajectory set $\mathcal{D}^{(r)}$.
%
We maintain an experience bank $\mathcal{B}^{(r)}$ containing all trajectories accumulated up to and including round $r$, including both successful and failed interactions:
\begin{equation}
\mathcal{B}^{(r)}
=
\mathcal{B}^{(r-1)} \cup \mathcal{D}^{(r)},
\qquad
\mathcal{B}^{(0)}=\emptyset.
\label{eq:experience_bank}
\end{equation}
%
Thus, $\mathcal{D}^{(r)}$ represents the newly collected on-policy experience at round $r$, while $\mathcal{B}^{(r)}$ provides the accumulated experience available for retrospective supervision in that round.

\paragraph{Privileged Retrospective Context.}
For each trajectory $\tau\in\mathcal{D}^{(r)}$ and interaction turn $i$, we construct turn-level privileged context
\begin{equation}
c_i^{(r)}
=
\mathcal{H}
\left(
P^{(r)},
L^{(r)},
R_i^{(r)},
F_i^{(r)}
\right),
\label{eq:privileged_context}
\end{equation}
where $P^{(r)}$ and $L^{(r)}$ are derived from accumulated historical experience, while $R_i^{(r)}$ and $F_i^{(r)}$ exploit information available after completing the current trajectory.

\textit{Precedents} $P^{(r)}$ provide concrete prior experiences that demonstrate useful behaviors for solving related tasks.
%
We first apply task-specific heuristics to identify useful trajectories from $\mathcal{B}^{(r)}$, rank the resulting candidates by content-token overlap with the current task goal, and retrieve the top-$n$ as precedents.
%
These precedents complement the current trajectory with transferable action patterns observed in previous interactions.

\textit{Lessons} $L^{(r)}$ provide a more abstract view of accumulated experience.
%
For each task type, we expose selected successful and failed experiences of that type from $\mathcal{B}^{(r)}$ to the current policy model and ask it to summarize reusable strategies and recurring failure patterns.
%
The lesson summary is generated once per task type and round; we suppress the task-type index for notational simplicity:
\[
L^{(r)}
=
\operatorname{Summarize}_{\pi^{(r)}}\!\left(\mathcal{B}^{(r)}\right).
\]
%
Unlike precedents, lessons compress experience into reusable abstractions and allow unsuccessful trajectories to contribute even when they are unsuitable as concrete demonstrations.

The remaining two components are constructed retrospectively from the current trajectory.
%
At each turn $i$, the current policy model produces a \textit{reflection}
\[
R_i^{(r)}
=
\operatorname{Reflect}_{\pi^{(r)}}(h_i,\tau),
\]
which uses the completed interaction to diagnose the realized decision and summarize what could have been done more effectively.
%
We further provide \textit{future hindsight}
\[
F_i^{(r)} = \tau_{>i},
\]
which directly exposes the downstream interaction following turn $i$, including subsequent environment feedback and outcome information.
%
Importantly, both $R_i^{(r)}$ and $F_i^{(r)}$ are constructed only after the trajectory is completed and are used exclusively for retrospective teacher re-scoring; they are never available to the acting policy during rollout.
%
Whereas reflection converts hindsight into an explicit assessment, future hindsight preserves the downstream evidence itself.
%
Together, these four components provide the teacher with both cross-task experience and within-trajectory hindsight that were unavailable to the acting policy at generation time. The exact generation prompts are provided in \appref{sec:prompt_templates}.

\paragraph{Retrospective Distillation.}
Given $c_i^{(r)}$, we optimize the student using the OPSD objective in Eq.~\ref{eq:opsd}.
%
For every action token $j$ at turn $i$, the teacher conditions on $(h_{i,j},c_i^{(r)})$, whereas the student observes only $h_{i,j}$.
%
The teacher retrospectively re-scores the student's realized trajectory rather than generating a replacement trajectory, thereby providing dense supervision directly over the states visited by $\pi^{(r)}$.
%
After distillation, the updated student becomes $\pi^{(r+1)}$ and is used to collect $\mathcal{D}^{(r+1)}$.

\paragraph{Self-Evolution Flywheel.}
The interaction between policy evolution and experience accumulation forms a recurrent data flywheel.
%
At each round, $\pi^{(r)}$ generates new trajectories $\mathcal{D}^{(r)}$, which expand the experience bank to $\mathcal{B}^{(r)}$ through Eq.~\ref{eq:experience_bank} and refresh the precedents $P^{(r)}$ and lessons $L^{(r)}$ used for retrospective supervision.
%
Meanwhile, each newly collected trajectory provides fresh reflection $R_i^{(r)}$ and future hindsight $F_i^{(r)}$ for its own retrospective supervision.
%
The resulting privileged context in Eq.~\ref{eq:privileged_context} is distilled back into the policy, closing the flywheel between model evolution, accumulated experience, and privileged retrospective supervision.

\subsection{Frontier-Guided Context-Policy Evolution}
\label{sec:frontier_method}

The self-evolution procedure above continually refreshes the contents of privileged context as new experience enters the bank, while keeping the context-construction rule $\mathcal{H}$ fixed.
%
However, the most useful way to construct privileged supervision may itself change as the agent evolves.
%
We therefore consider a stronger-access setting that assumes access to both a frontier model and an executable verifier or environment metric, and uses them to optimize the context-construction policy.
%
The verifier is used only to evaluate context-policy candidates and their realized post-training performance; it does not provide rewards for optimizing the agent parameters, which continue to be updated solely through OPSD.

We parameterize the privileged-context constructor by a context policy $\phi^{(r)}$,
\begin{equation}
c_i^{(r)}
=
\mathcal{H}_{\phi^{(r)}}
\left(
P^{(r)},
L^{(r)},
R_i^{(r)},
F_i^{(r)}
\right),
\label{eq:context_policy}
\end{equation}
where $\phi^{(r)}$ controls how these information sources are selected and composed.
%
We represent $\phi^{(r)}$ as a declarative configuration over a constrained set of editable choices, including precedent count and retrieval strategy, lesson usage, reflection, future hindsight, the position at which privileged information is injected into the teacher context, and a small set of teacher-side re-scoring settings such as temperature.
%
The frontier model may modify only these whitelisted configuration choices, without modifying the model weights or training procedure.

\paragraph{Frontier-Guided Proposal.}
After completing evolution round $r$, the frontier model receives a compact summary of the current training state, including the current context policy, checkpoint task performance, and teacher re-scoring statistics such as correction rate, teacher entropy, and top-$k$ hit rate, with detailed definitions in \appref{sec:teacher_diagnostics}.
%
Based on these diagnostics, it proposes a small set of candidate edits to $\phi^{(r)}$.
%
To ground this search in empirical feedback, each candidate is evaluated with a lightweight no-training probe: we instantiate the candidate privileged context on a small training-distribution slice, provide it to the current model at inference time, and measure the corresponding task performance without updating model parameters.
%
The frontier model observes these probe scores and selects a candidate $\tilde{\phi}^{(r+1)}$ for the subsequent self-evolution round.

\paragraph{Retrospective Acceptance.}
The selected candidate $\tilde{\phi}^{(r+1)}$ is then used to construct privileged supervision during the subsequent full self-evolution round.
%
After training, we evaluate the resulting checkpoint using the actual environment metric.
%
The proposed context policy is retained if its post-training performance is no worse than the best previously accepted configuration (up to a tolerance $\epsilon$); otherwise, the context policy reverts to the last accepted configuration:
\begin{equation}
\phi^{(r+1)}
=
\begin{cases}
\tilde{\phi}^{(r+1)}, & m^{(r+1)} \geq m_{\mathrm{best}}^{(r)}-\epsilon,\\
\phi_{\mathrm{best}}^{(r)}, & \text{otherwise},
\end{cases}
\label{eq:context_acceptance}
\end{equation}
where $m^{(r+1)}$ denotes the realized post-training environment performance.
%
Only the context policy is reverted; the model parameters continue evolving across rounds.

\paragraph{Joint Evolution of Model and Context Policy.}
The frontier-guided extension therefore adds a second adaptive process to the self-evolution flywheel.
%
The core procedure evolves the model and the privileged information available from accumulated experience, while frontier guidance additionally evolves how that information is selected and organized:
\[
\pi^{(r)} \rightarrow \pi^{(r+1)},
\qquad
\mathcal{B}^{(r)} \rightarrow \mathcal{B}^{(r+1)},
\qquad
\phi^{(r)} \rightarrow \phi^{(r+1)}.
\]
%
This allows the retrospective supervision mechanism itself to adapt to the evolving agent rather than relying on a single hand-designed context policy throughout training.

==> neurips_sections/5_experiments.tex <==
\section{Experiments}\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:setup}

\paragraph{Models.}
We conduct experiments with Qwen3-8B and Qwen3-14B~\citep{yang2025qwen3} as the base agent models to study self-evolution across model scales.
%
For frontier-guided context-policy evolution, we use Claude-Opus-4.8~\citep{anthropic2026claudeopus48} as the frontier model that proposes constrained modifications to the privileged harness configuration.
%
We access Claude through OpenCode~\citep{opencode2026}, which serves as the coding and orchestration harness for generating and applying the proposed configuration edits.

\paragraph{Benchmarks and Evaluation Metrics.}
We evaluate \ours on three agent benchmarks: ALFWorld~\citep{shridhar2020alfworld}, ScienceWorld~\citep{wang2022scienceworld}, and SearchQA~\citep{jin2025search}.
%
Together, these benchmarks span embodied household interaction, scientific reasoning and environment manipulation, and search-based question answering, providing diverse settings for evaluating iterative agent self-evolution.
%
For ALFWorld, we report success rate (SR) on the valid seen and valid unseen splits.
%
For ScienceWorld, we report task success rate (SR) on the development set.
%
For SearchQA, we report exact match (EM).
%
Additional evaluation details are provided in \appref{sec:implementation_details}.

\paragraph{Baselines.}
We compare \ours against several representative adaptation and self-improvement baselines.
%
Base model (Base) directly evaluates the pretrained agent without additional adaptation, while Rejection sampling Fine-Tuning (RFT)~\citep{yuan2023scaling} fine-tunes the model on its own successful trajectories.
%
Ground-Truth Supervised Fine-Tuning (GT-SFT) provides an oracle-supervision reference by fine-tuning on ground-truth trajectories, while Self-Taught Reasoner (STaR)~\citep{zelikman2022star} iteratively improves the model using self-generated successful trajectories.
%
We further compare against Group Relative Policy Optimization (GRPO)~\citep{shao2024deepseekmath}, which performs verifier-based reinforcement learning when an executable reward is available, and Ground-Truth On-Policy Self-Distillation (GT-OPSD)~\citep{zhao2026self}, which replaces our privileged context with gold-reference agent trajectories during distillation.
%
Moreover, we include Harness-at-Inference (Harness@Inf), which directly supplies the privileged context to the base model without post-training.

\paragraph{Implementation Details.}
We run self-evolution for 10 rounds, sampling 200 unique training instances in each round, and optimize the model using full-parameter forward-KL distillation with a learning rate of $3\times10^{-6}$.
%
Unless otherwise specified, \ours is evaluated using the evolved student alone without privileged context at inference time; additional training, decoding, and task-specific implementation details are provided in \appref{sec:implementation_details}.

\subsection{Main Results}
\label{sec:main_results}


\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{\textbf{ALFWorld (SR)}}
& \multicolumn{2}{c}{\textbf{ScienceWorld (SR)}}
& \multicolumn{2}{c}{\textbf{SearchQA (EM)}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\textbf{Method}
& \textbf{Qwen3-8B} & \textbf{Qwen3-14B}
& \textbf{Qwen3-8B} & \textbf{Qwen3-14B}
& \textbf{Qwen3-8B} & \textbf{Qwen3-14B} \\
\midrule

Base
& 62.9 & 69.3
& 15.6 & 12.9
& 35.4 & 35.4 \\

RFT
& 66.9 & 71.0
& 12.7 & 14.3
& 35.4 & 36.3 \\

GT-SFT
& 34.1 & 42.7
& 11.6 & 13.4
& 34.7 & 35.2 \\

STaR
& 65.3 & 77.8
& 12.7 & 13.6
& 34.4 & 37.6 \\

GRPO
& \underline{75.5} & \textbf{82.6}
& -- & --
& 37.3 & 37.3 \\

GT-OPSD
& 70.1 & \underline{82.5}
& 3.0 & 3.0
& 37.1 & 38.5 \\

Harness@Inf
& 65.4 & 72.0
& \underline{19.6} & \underline{20.5}
& \underline{37.7} & \textbf{41.4} \\

\textbf{\ours}
& \textbf{76.6} & 79.6
& \textbf{23.4} & \textbf{20.6}
& \textbf{37.9} & \underline{38.7} \\

\bottomrule
\end{tabular}
\caption{
Main results across ALFWorld, ScienceWorld, and SearchQA.
For ALFWorld, SR is averaged over the valid-seen and valid-unseen splits, while for SearchQA, EM is averaged across the evaluated sub-datasets.
Results for \ours are averaged over three seeds.
\textbf{Bold} denotes the best result and \underline{underline} denotes the second-best result in each setting.
}
\label{tab:main_results}
\end{table}


\label{sec:main_results}

\tabref{tab:main_results} summarizes the main results across three benchmarks and two model scales.
%
Overall, \ours consistently improves over the corresponding base models and outperforms the self-training baselines in most settings.
%
On ALFWorld-8B, \ours achieves the best overall performance with an average SR of 76.6, compared with 62.9 for Base, 66.9 for RFT, and 65.3 for STaR.
%
The gains are particularly pronounced on ScienceWorld, where \ours improves from 15.6 to 23.4 at 8B and from 12.9 to 20.6 at 14B, while RFT, GT-SFT, and STaR provide little or no improvement.
%
This suggests that simply training on successful or oracle trajectories is insufficient in challenging interactive environments, whereas retrospectively supervising the agent on its own on-policy state distribution provides a more effective learning signal.
%
In contrast, SearchQA exhibits a relatively narrow performance range across methods.
%
Our later analyses provide a consistent picture: performance remains largely flat across self-evolution rounds (\figref{fig:self_evolution_curves}), teacher corrections remain moderate but comparatively stable (\appref{sec:teacher_diagnostics}), and privileged context retains inference-time utility without being effectively internalized into the evolved model (\figref{fig:harness_internalization}).
%
This suggests that the SearchQA boundary case reflects limited capacity to convert the available retrospective signal into persistent behavioral improvement, rather than simply an absence of useful contextual information.

\paragraph{Comparison with Reward-Driven and Oracle Baselines.}
\ours remains competitive with methods that rely on substantially stronger supervision.
%
On ALFWorld-14B, GRPO and GT-OPSD achieve 82.6 and 82.5 SR, respectively, compared with 79.6 for \ours.
%
However, GRPO relies on environment rewards and multiple grouped rollouts for policy optimization, substantially increasing rollout cost, while GT-OPSD explicitly conditions the teacher on a ground-truth successful agent trajectory.
%
In contrast, \ours learns from the agent's own interaction experience through privileged retrospective context, without requiring oracle demonstrations or reward-driven group optimization.
%
Notably, \ours achieves the best result on ALFWorld-8B and substantially outperforms the supervised baselines on ScienceWorld at both model scales.

\paragraph{Beyond Inference-Time Harnessing.}
We further compare against Harness@Inf, which directly provides the privileged context to the base model during inference without updating model parameters.
%
\ours matches or exceeds Harness@Inf in five of the six model--benchmark settings, with particularly clear improvements on ALFWorld and ScienceWorld-8B.
%
For example, ALFWorld-8B improves from 65.4 with Harness@Inf to 76.6 after self-evolution, while ScienceWorld-8B improves from 19.6 to 23.4.
%
These results indicate that the benefit of privileged context is not limited to inference-time scaffolding: iterative self-evolution can transfer useful information from the harness into the model itself.
%
We further investigate how the privileged context evolves across self-evolution rounds in \secref{sec:context_evolution}.
%
SearchQA-14B provides an important boundary case, where Harness@Inf reaches 41.4 compared with 38.7 for \ours, suggesting that some contextual information remains complementary to the model rather than being fully internalized.

\subsection{Self-Evolution Across Rounds.}
\label{sec:self_evolution_analysis}



\figref{fig:self_evolution_curves} shows representative self-evolution trajectories over ten rounds for both model scales.
%
On ALFWorld, both Qwen3-8B and Qwen3-14B progressively reach substantially higher success rates than their initial models and the RFT baselines, although improvement is not strictly monotonic across rounds.
%
A similar pattern emerges on ScienceWorld: performance initially fluctuates around the baseline but improves noticeably in later rounds, indicating that useful behaviors can accumulate gradually through repeated self-evolution.
%
In contrast, SearchQA remains within a relatively narrow performance band throughout training, consistent with the limited gains observed in Table~\ref{tab:main_results}.
%
Additional teacher re-scoring diagnostics show a similarly stable correction signal (\appref{sec:teacher_diagnostics}).
%
Together, these trajectories show that repeated self-evolution can progressively improve interactive agent behavior on ALFWorld and ScienceWorld, while also revealing that the effectiveness of self-evolution depends on whether the task provides learnable behavioral headroom.
%
We next investigate which components of the privileged context enable this improvement and how the resulting supervision is transferred across evolution rounds.
%
Additional teacher re-scoring diagnostics, including task-specific correction profiles are provided in \appref{sec:teacher_diagnostics}.


==> neurips_sections/6_analysis.tex <==
\section{Analysis}\label{sec:generalization}

\subsection{Ablation Studies}
\label{sec:ablation}
\begin{wraptable}{r}{0.45\textwidth}
    \centering
    \small
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Variant} & \textbf{ALFWorld SR} & \textbf{ScienceWorld SR} \\
    \midrule
    Full              & 76.6 & 23.4 \\
    $-$ Precedents    & 75.0 & 15.1 \\
    $-$ Lessons & 71.6 & 22.7 \\
    $-$ Reflection    & 71.4 & 21.8 \\
    $-$ Future        & 71.4 & 17.6 \\
    \bottomrule
    \end{tabular}
    \caption{
    Ablation of privileged-context components on Qwen3-8B.
    }
    \label{tab:context_ablation}
\end{wraptable}

\tabref{tab:context_ablation} studies the contribution of different components in the privileged context.
%
On ALFWorld, removing lessons, reflection, or future hindsight
each reduces SR by roughly five points, while removing precedents has only a minor effect.
%
ScienceWorld exhibits a different pattern: removing precedents decreases SR from 23.4 to 15.1, nearly returning to the Base performance of 15.6, while removing future also causes a substantial drop to 17.6.
%
In comparison, lessons and reflection provide smaller gains on ScienceWorld.
%
To examine the source of the lesson signal, we construct lessons from successful or failed trajectories only.
%
Restricting lessons to either successful or failed trajectories yields lower performance than the default main-result reference, suggesting that both sources may provide useful retrospective information (\appref{sec:lesson_source_ablation}).
%
These results indicate that different environments benefit from different forms of privileged information, with trajectory-specific hindsight being more important on ALFWorld and transferable precedents being important on ScienceWorld.

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{7pt}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Variant} & \textbf{ALFWorld SR} & \textbf{ScienceWorld SR} \\
% \midrule
% Full              & 76.6 & 23.4 \\
% $-$ Precedents    & 75.0 & 15.1 \\
% $-$ Lessons & 71.6 & 22.7 \\
% $-$ Reflection    & 71.4 & 21.8 \\
% $-$ Future        & 71.4 & 17.6 \\
% \bottomrule
% \end{tabular}
% \caption{
% Ablation of privileged-context components on Qwen3-8B.
% Different tasks rely on different privileged signals: generated hindsight components dominate on ALFWorld, whereas precedents are essential on ScienceWorld.
% }
% \label{tab:context_ablation}
% \end{table}




\subsection{Effect of Context Evolution}
\label{sec:context_evolution}

We next examine whether evolving the privileged context with newly collected experience is itself important for continued self-evolution.
%
Starting from the same base checkpoint, we train each variant for three self-evolution rounds and compare the standard evolving-context configuration of \ours against variants that evolve only lessons, evolve only precedents, or freeze the round-1 context for all subsequent rounds.
%
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/opsd_exp1_context_evolution_alfworld.pdf}
    \vspace{-0.3in}
    \caption{
    Context evolution on ALFWorld-8B.
    Refreshing privileged context across self-evolution rounds substantially outperforms freezing the round-1 context, with lesson updates providing particularly strong gains.
    }
    \label{fig:context_evolution}
    \vspace{-0.5in}
\end{wrapfigure}
As shown in \figref{fig:context_evolution}, all variants begin from the
same performance at round 0, while their trajectories increasingly diverge as different context updates accumulate.
%
By round 3, the full evolving-context configuration reaches $67.9\%$ unseen SR, while refreshing lessons alone reaches $69.0\%$ and refreshing precedents alone reaches $63.8\%$; in contrast, freezing the round-1 context drops to $59.7\%$.
%
This suggests that, on ALFWorld, refreshing generated retrospective information is particularly important, consistent with the component ablation in \tabref{tab:context_ablation}.
%
Overall, these results show that repeatedly training against stale retrospective context limits continued improvement, whereas refreshing the context with newly collected experience supports continued self-evolution.



\subsection{Frontier-Guided Context-Policy Evolution}
\label{sec:frontier_context}

We next study a stronger-access extension in which privileged-context construction is itself optimized by a frontier model.
%
In this setting, we assume access to both a frontier model and an executable environment metric, which together enable an outer-loop search over context-construction policies.
%
At each round, the frontier model proposes a small YAML edit to the privileged-context policy from a constrained whitelist of editable knobs.
%
Candidate selection is performed using a cheap no-training privileged-context-at-inference probe, while retrospective acceptance or rejection is determined only after a full self-evolution round using the realized environment performance.
%
We compare this frontier-guided setting against two controls: \textit{Fixed}, which keeps the canonical privileged-context policy unchanged throughout training, and \textit{Random}, which explores the same edit space under the same edit budget but without frontier guidance.

\paragraph{Frontier Guidance Improves Context Evolution.}
As shown in \figref{fig:frontier_context_results}, frontier-guided context-policy evolution yields the clearest gains on ScienceWorld, where it improves SR from 23.4 to 27.5 at 8B and from 20.6 to 29.8 at 14B relative to the fixed policy, and also outperforms random search at both scales.
%
On ALFWorld, the gains are smaller but still positive, with SR improving from 76.6 to 78.4 at 8B and from 79.6 to 80.3 at 14B.
%
This pattern suggests that frontier-guided context optimization is most useful when privileged-context construction has substantial headroom, while remaining competitive in the more saturated ALFWorld regime.
%
We therefore focus the frontier-guided study on ALFWorld and ScienceWorld, where the preceding analyses reveal clearer self-evolution and context-construction headroom.
%
SearchQA serves instead as a complementary boundary case, where self-evolution remains limited and privileged context shows little evidence of persistent internalization into the model (\figref{fig:harness_internalization}; Appendix~\ref{sec:teacher_diagnostics}).




==> neurips_sections/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We study self-evolving language agents that improve from their own on-policy interaction experience without requiring ground-truth trajectories or verifier-derived rewards for the core policy update.
%
We introduce \ours, which constructs privileged retrospective context from accumulated experience and trajectory hindsight, and distills this richer view back into the policy through on-policy self-distillation.
%
Across multiple agent benchmarks and model scales, \ours consistently improves over the corresponding base models.
%
Our ablation and context-evolution analyses further show that different privileged signals contribute complementary information and that continually refreshing the retrospective context is important for sustained self-evolution.
%
We additionally introduce frontier-guided context-policy evolution, allowing the construction of privileged supervision itself to adapt as the agent evolves.
%
Together, these results demonstrate a practical data flywheel in which model capability, accumulated experience, and retrospective supervision improve jointly across rounds.



==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}



==> sections/2_related.tex <==
\section{Related Work}
\label{sec:related}



==> sections/3_prelim.tex <==
\section{Preliminaries}\label{subsec:preliminaries}

==> sections/4_method.tex <==
\section{\ours}\label{sec:workflow}


==> sections/5_experiments.tex <==
\section{Experiments}\label{sec:experiments}


==> sections/6_analysis.tex <==
\section{Analysis}\label{sec:generalization}


==> sections/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

